Towards a new paradigm of scientific discovery with socialized artificial intelligence

Scientific discovery has advanced through successive transformations in the organization of knowledge. Observation and experimentation established the empirical foundations of science. Theory made it possible to derive general principles from particular phenomena. Computation extended inquiry into systems beyond direct observation, while data-intensive methods opened new spaces of pattern and prediction. Science now confronts a different frontier. The central challenge is no longer simply to produce more information, but to organize expanding knowledge, reasoning, and evidence into a coherent process of discovery. Here, we introduce Bridging Literature, Agents, and Zero-gap Experimentation (BLAZE), a paradigm of socialized scientific intelligence. BLAZE conceives AI not as an assistant for isolated research tasks, but as an organizational infrastructure for scientific discovery. It connects persistent knowledge, collective reasoning, empirical validation, and human judgment within a continuous research lifecycle, transforming fragmented activities into a cumulative process of inquiry, criticism, and revision. The central premise of BLAZE is that scientific intelligence does not arise from computation alone. It emerges from the sustained interaction among knowledge, hypotheses, experiments, and collective verification. By organizing humans and machines within a shared scientific process, BLAZE makes discovery more traceable, reproducible, and cumulative while preserving human creativity, judgment, and responsibility. Socialized scientific intelligence may provide a foundation for the next era of science. Its purpose is not to replace human discovery, but to extend the scale, depth, and continuity of collective scientific inquiry.

==> 3-BLAZE_Research_System/3.tex <==
\section{BLAZE Research System: A Socialized AI4R Architecture}
\label{sec:system}

End-to-end research automation is often formulated as a sequence of isolated capabilities: retrieving literature, proposing an idea, executing code and generating a manuscript~\cite{lu2024aiscientist}. Such a formulation, however, overlooks the organizational structure that makes scientific research reliable. A plausible hypothesis must be grounded in prior knowledge, an experiment must be traceable to the hypothesis that motivated it, and each reported claim must remain connected to the evidence from which it was derived. Scientific output must also be open to criticism, revision and ultimately human accountability~\cite{marusic2010singapore}.

Here we present the BLAZE Research System, a socially organized AI-for-research infrastructure that coordinates knowledge, specialized research agents, executable tools and human governance across the scientific life cycle. Rather than treating a paper as the terminal output of a linear pipeline, BLAZE models research as a recurrent process in which hypotheses, experiments, reviews and revisions continuously update a shared body of knowledge. The system therefore aims not merely to automate individual research tasks, but to organize how research questions are formulated, tested, challenged, communicated and retained.

\subsection{The BLAZE Research Lifecycle}
\label{sec:lifecycle}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.92\linewidth]{figures/BLAZE-lifecycle.png}
    \caption{Overview of the BLAZE research workflow.}
    \label{fig:blaze-lifecycle}
\end{figure}

BLAZE organizes a research project into eleven connected stages (Fig.~\ref{fig:blaze-lifecycle}): topic specification, knowledge-base construction, research-landscape analysis, gap mining, socialized hypothesis generation, research-plan compilation, experiment-graph execution, evidence-constrained manuscript generation, human-AI review, revision and additional experimentation, and knowledge sedimentation.

The process begins with a research topic supplied by a human scientist. In addition to a textual description, the input may include disciplinary boundaries, available datasets and instruments, computational budgets, expected forms of contribution and explicit safety constraints. These specifications define the scope of the project rather than predetermine its scientific conclusion. BLAZE subsequently constructs a project-specific knowledge context by combining broadly accessible scientific literature with private materials supplied by the research team, such as unpublished observations, previous experiments, internal reports and reviewer feedback.

From this context, the system produces a research dashboard that summarizes the structure of the field, including major questions, representative methods, commonly used datasets, influential research groups, emerging trends and unresolved disagreements. Gap mining is then performed over this structured landscape. Candidate gaps are not represented as free-form statements alone; each is accompanied by the literature from which it was inferred, the limitations of existing approaches, potentially conflicting evidence and an assessment of whether the gap is scientifically meaningful and experimentally addressable.

These candidates are passed to the socialized hypothesis-generation stage. Specialized agents propose, criticize and revise possible explanations or methodological directions. The resulting hypotheses are evaluated according to novelty, scientific relevance, falsifiability, feasibility and expected value. A selected hypothesis is subsequently compiled into a research plan that specifies the experimental variables, baselines, controls, ablations, datasets, evaluation criteria, statistical tests, resource requirements and stopping conditions. This compilation step is important because it transforms a linguistically plausible idea into an executable and falsifiable research object.

The plan is represented as an experiment graph, in which nodes correspond to executable operations and edges encode dependencies between them~\cite{moreau2013prov}. Nodes may include data preparation, baseline reproduction, method implementation, debugging, hyperparameter exploration, ablation, replication, statistical analysis and visualization. Failed executions do not disappear from the workflow. Instead, they generate diagnostic nodes and become part of the project history, allowing subsequent agents to distinguish unsupported hypotheses from implementation failures.

Experimental outputs are then incorporated into a shared evidence structure. Numerical results, plots, configuration files, code versions and statistical analyses are linked to the hypotheses and claims that they support or contradict. Manuscript generation operates on this evidence structure rather than directly on unconstrained model memory. Statements lacking sufficient evidence are marked for qualification, additional experiments or removal.

The resulting manuscript is assessed by both AI reviewers and human researchers. Reviews are converted into structured revision tasks, such as correcting an implementation, adding a control group, weakening an unsupported claim or clarifying the relation to previous work. Tasks requiring new evidence are returned to the experiment graph, creating a revision loop rather than a purely textual editing stage. After review and revision, the project's literature annotations, hypotheses, negative results, successful experiments, reviewer disagreements and final conclusions are deposited back into the knowledge base. Thus, the terminal state of one project becomes part of the initial scientific memory of the next.

Quality control is applied at the transitions between stages. A candidate hypothesis must pass novelty and feasibility checks before plan compilation; an experiment must satisfy execution and reproducibility criteria before its results can support a claim; and a manuscript must pass evidence, ethical and authorship checks before external dissemination. When a gate is not satisfied, the system routes the project back to the stage at which the missing evidence or unresolved risk originated.

\subsection{Four-Layer System Architecture}
\label{sec:four-layer-architecture}

The BLAZE architecture comprises four interacting layers: the knowledge and memory layer, the agent society layer, the tool and execution layer, and the evaluation and governance layer (Fig. 3b). The separation between these layers allows scientific reasoning, task execution and quality control to evolve independently while remaining connected through shared research artefacts.

The knowledge and memory layer provides the factual and historical context of the project~\cite{wilkinson2016fair}. It contains public scientific knowledge, user-authorized private collections, structured relations between scientific entities, experimental records, manuscript versions and previous review histories. It supports both semantic retrieval and relational queries over papers, authors, institutions, tasks, methods, datasets, claims and evidence. Importantly, this layer stores not only successful conclusions but also failed experiments, disputed interpretations and unresolved questions. Such records reduce repeated exploration and help the system reason about why a direction was previously abandoned or remained inconclusive.

The agent society layer performs scientific reasoning and coordination. Instead of assigning the entire project to a single general-purpose model, BLAZE distributes responsibilities among agents with distinct scientific roles~\cite{wu2023autogen}. These agents interpret knowledge, formulate questions, design methods, challenge assumptions, execute experiments, assess uncertainty and organize scientific communication. A coordinating principal-investigator agent maintains the project-level objective and reconciles competing recommendations, but does not replace the specialized judgement of the other agents.

The tool and execution layer converts research decisions into observable operations. It provides literature-retrieval interfaces, code repositories, data-processing environments, notebook and container execution, statistical-analysis packages, visualization tools, document compilers and, where appropriate, interfaces to external scientific instruments. Executions are isolated, logged and versioned so that outputs can be traced to the code, data, parameters and environment that produced them. The same abstraction can accommodate both computational experiments and future physical-laboratory operations, although actions involving physical instruments require additional safety and authorization mechanisms.

The evaluation and governance layer operates across the complete architecture. It performs novelty checking, evidence verification, reproducibility assessment, statistical validation, automated peer review, ethical screening and permission control. It also records which decisions were made autonomously, which were suggested by AI but approved by humans, and which were overridden. This provenance makes it possible to audit not only the final manuscript but also the process through which its scientific claims were produced.

Communication between layers is mediated by structured research artefacts rather than unrecorded conversational context. Examples include literature matrices, gap reports, hypothesis cards, experiment specifications, execution logs, statistical reports, claim-evidence links and review records. Each artefact has a defined origin, version and status. This design enables one agent to inspect or challenge the work of another and prevents unsupported statements from silently propagating between stages.

\subsection{Agent Society: From a Single Model to a Research Community}
\label{sec:agent-society}

BLAZE treats multi-agent research as an organizational problem rather than a role-playing exercise. Each agent is defined by a research responsibility, an input and output schema, permitted tools, evaluation criteria and a stopping condition~\cite{hong2024metagpt}. The agent society is intended to approximate the functional diversity of a research group, in which scientific progress emerges from division of labour, disagreement and repeated scrutiny.

The PI Agent maintains the global research objective, allocates tasks and adjudicates major conflicts. The Literature Agent retrieves and organizes prior work, identifies relevant evidence and evaluates whether a proposed contribution overlaps with existing studies. The Domain Expert Agent checks disciplinary assumptions, practical constraints and scientific plausibility. The Methodologist Agent translates research gaps into candidate models, mechanisms or analytical strategies.

Critical assessment is provided by the Skeptic Agent, which searches for hidden assumptions, counterexamples, confounding variables and alternative explanations. Its purpose is not simply to lower an idea score, but to produce concrete tests capable of distinguishing a genuine contribution from an artefact. The Experiment Agent converts approved plans into executable code and maintains the experiment graph, whereas the Statistician Agent evaluates uncertainty, replication consistency, effect size and statistical significance. The Writer Agent organizes the validated evidence into a manuscript, and the Reviewer Agent evaluates the resulting work against venue- or domain-specific criteria. An Ethics Agent examines data use, disclosure, attribution, dual-use concerns and other risks throughout the process.

Scientific deliberation follows a propose-challenge-revise-adjudicate cycle. Agents initially produce independent analyses to reduce premature convergence. Critiques must identify the claim being challenged and, where possible, cite evidence or propose a discriminating experiment. The hypothesis owner then revises or defends the proposal, after which the PI Agent determines whether the idea should be accepted, rejected, archived or returned for further investigation.

Disagreement is retained as scientific information. When agents reach different conclusions because the available evidence is insufficient, BLAZE records the competing interpretations and converts the disagreement into an experimental question. This mechanism reduces the risk of an agent echo chamber, in which apparent consensus results from shared model biases rather than convergent evidence. The system therefore values productive conflict: disagreement should either reveal a flaw or generate a test capable of resolving it.

Agents are activated dynamically rather than uniformly. A straightforward literature query may require only a literature specialist, whereas a claim involving uncertain measurements may invoke a domain expert, statistician and skeptic. This selective organization limits unnecessary communication and computational cost while preserving multidisciplinary scrutiny for consequential decisions.

\subsection{Human Governance and Intervention Points}
\label{sec:human-governance}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.92\linewidth]{figures/Human governance checkpoints.png}
    \caption{Human oversight points embedded in the BLAZE workflow.}
    \label{fig:human-governance-checkpoints}
\end{figure}

BLAZE is designed as a human-AI collaborative research infrastructure, not as an autonomous publication machine~\cite{wickramasinghe2020trustworthy}. Human responsibility is preserved through five mandatory checkpoints (Fig.~\ref{fig:human-governance-checkpoints}): topic approval, hypothesis approval, experiment approval, submission approval, and ethics and authorship approval.

At topic approval, researchers determine whether the proposed project is scientifically meaningful, appropriately scoped and compatible with available resources. At hypothesis approval, humans inspect the supporting literature, novelty analysis, anticipated contribution and major objections raised during agent deliberation. This prevents a highly scored but scientifically trivial or socially inappropriate idea from entering the experimental stage.

Experiment approval is required before substantial computational resources, sensitive datasets or physical instruments are used. Researchers can modify baselines, controls, budgets and stopping criteria, and may prohibit actions that create unacceptable technical, ethical or financial risks. Submission approval occurs only after humans inspect the manuscript, evidence links, reproduction package and unresolved reviewer concerns. BLAZE does not treat an automatically generated acceptance recommendation as authorization to submit.

The final checkpoint covers ethics and authorship. Human researchers must confirm appropriate attribution, disclosure of AI involvement, data permissions, conflict-of-interest statements and responsibility for the scientific claims. Authorship cannot be inferred solely from agent participation; accountable humans must determine who satisfies the relevant contribution and responsibility standards.

At each checkpoint, the system exposes the evidence and uncertainty underlying its recommendation. Humans can accept, revise or reject the proposed transition, and their decisions are retained in the project record. High-risk actions can also be configured to require multiple independent approvals. These mechanisms ensure that increasing automation does not weaken scientific accountability.

By combining a recurrent research lifecycle, layered execution architecture, differentiated agent society and explicit human governance, BLAZE shifts the objective of AI4R from automating paper production to organizing accountable scientific discovery. Its central output is therefore not only a manuscript, but also a traceable research process in which questions, decisions, experiments, evidence and revisions remain connected.

==> 9-Comparative_Evaluation/9.1.tex <==
\setcounter{section}{8}
\section{Comparative Evaluation and Competitor Analysis}
\label{sec:evaluation}

This chapter evaluates BLAZE using shared task protocols, frozen delivery packages, and auditable execution records. Heterogeneous domain projects are treated as case studies, while controlled results are reported separately from test-feedback optimization.

\subsection{Evaluation Scope and Controls}
\label{sec:evaluation-scope}

The evaluation contains three tracks. The free-form track starts from a shared baseline and assesses whether a system delivers a traceable research package from reproduction to review. H-EDML uses a common five-dataset protocol to examine reproduction and score optimization. Task-specific tuning measures gains over local clean baselines and gaps to external references. Because model families and total computational budgets were not equalized across all systems, these tracks support evidence-level comparison rather than a causal attribution of research quality to BLAZE.

\begin{table}[h]
\centering
\caption{Evaluation tracks and interpretation.}
\label{tab:evaluation-tracks}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}llp{0.47\linewidth}@{}}
\toprule
\textbf{Track} & \textbf{Control} & \textbf{Valid use and limit} \\
\midrule
Free-form & Baseline & Delivery/audit; no cross-task rank \\
H-EDML & 5 datasets & Reproduction/tuning; no causal claim \\
Task tuning & Clean baseline & Local gain; no held-out claim \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Frozen-Package Competitor Evaluation}
\label{sec:package-evaluation}

Three independent GPT reviewers scored identical frozen delivery packages using a 100-point rubric. The rubric assigns 15 points each to protocol alignment, lifecycle coverage, and experimental rigor; 20 points to traceability; 10 points each to claim calibration and final research output; 5 points to resource disclosure; and 10 points to quantitative breadth. The score measures the completeness and auditability of the submitted evidence rather than scientific impact or the theoretical capability ceiling of each system. All three reviewers produced the same ranking, yielding Kendall's $W=1.00$.

\begin{table}[h]
\centering
\caption{Frozen-package scores from three independent GPT reviewers.}
\label{tab:package-scores}
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{lrrrr}
\toprule
\textbf{System} & \textbf{R1} & \textbf{R2} & \textbf{R3} & \textbf{Mean $\pm$ SD} \\
\midrule
AutoPaper & 91 & 96 & 98 & $\mathbf{95.0 \pm 3.6}$ \\
ARIS & 90 & 95 & 94 & $\mathbf{93.0 \pm 2.6}$ \\
FARS & 46 & 45 & 38 & $43.0 \pm 4.4$ \\
EvoScientist & 13 & 12 & 21 & $15.3 \pm 4.9$ \\
\bottomrule
\end{tabular}
\end{table}

AutoPaper and ARIS form the same leading tier: their two-point mean difference is smaller than the observed reviewer dispersion. AutoPaper provides stronger cross-stage synthesis, claim control, and final-package organization, whereas ARIS preserves a particularly detailed raw experiment ledger. The lower FARS and EvoScientist scores describe the evidence visible in the frozen local packages, including incomplete process records or unfinished task delivery, rather than an absolute judgment of their underlying systems.

\subsection{Task-, Process-, and Cost-Level Evidence}
\label{sec:quantitative-evidence}

Under H-EDML, AutoPaper retained 162 auditable runs across five datasets. Its controlled A1 macro average was 83.09, while the higher value of 87.454 resulted from per-dataset test-feedback selection and is reported separately. ARIS completed all 50 planned runs across the same five-dataset protocol, although all five results remained below the corresponding paper values. Across five task-specific targets with aligned external references, AutoPaper reached or exceeded two, giving an attainment rate of 40\%.

\begin{table}[h]
\centering
\caption{Quantitative task evidence. TF denotes test-feedback selection.}
\label{tab:task-evidence}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
\textbf{Evidence} & \textbf{Datasets} & \textbf{Runs/Seeds} &
\textbf{Controlled} & \textbf{Optimized/Outcome} & \textbf{Reference result} \\
\midrule
AutoPaper H-EDML & 5 & 162 & 83.09 & 87.454 (TF) & $+2.718$ vs.\ 84.736 \\
ARIS H-EDML & 5 & 50/50 & -- & $5/5 < \mathrm{Ref.}$ & $0/5$ attained \\
Aligned external targets & 5 & -- & -- & $2/5$ attained & 40\% \\
AutoPaper PCS & 1 & 36 seeds & AUROC 1.000 & Spearman 0.8705 & constant-$B$ \\
\bottomrule
\end{tabular}%
}
\end{table}

The controlled and feedback-optimized H-EDML values answer different questions: 83.09 represents the stable comparison, whereas 87.454 demonstrates search capacity under disclosed test feedback. The 40\% external-reference attainment rate shows that the system can improve local reproductions and occasionally exceed reported references, but the outcome is mixed rather than uniformly state of the art. The PCS result provides repeated-run evidence for a scoped constant-$B$ claim and retains weaker NoRA and JLS alternatives as part of the research record.

Beyond task scores, AutoPaper completed 124 manuscript checks, rejected $2/3$ candidate ideas, and received an internal PCS review score of $7.2/10$. ARIS retained 950 raw experiment records and partial resource logs, including 3 GPUs for 34 minutes in B4 and 4 GPUs in B2. The available cost records also show that optimization is not free: ID73 required a $3.97$--$8.00\times$ runtime increase, while EvoScientist recorded 40.66 hours of wall-clock activity.

\subsection{Interpretation and Evidence Boundaries}
\label{sec:benchmark-limitations}

The present evidence supports two bounded conclusions. First, AutoPaper and ARIS provide the strongest auditable delivery packages among the four evaluated submissions, with complementary strengths in cross-stage integration and raw experiment traceability. Second, AutoPaper demonstrates reproducible score optimization across several tasks, but its external-reference results are mixed and several best values use explicitly disclosed test feedback. The evidence therefore supports auditable research delivery, negative-result retention, and protocol-bounded optimization; it does not establish that BLAZE universally produces higher-quality science or dominates specialized research systems.


==> 9-Comparative_Evaluation/9_old.tex <==
\setcounter{section}{8}
\section{Comparative Evaluation and Competitor Analysis}
\label{sec:evaluation}

BLAZE is evaluated as a research infrastructure that preserves inspectable links from scientific knowledge to hypotheses, executable studies, manuscript claims, and review-driven revisions. The evidence combines publication-grounded competitor analysis with local experiment records, review artifacts, audit trails, and four cross-domain cases. The evaluation emphasizes lifecycle coverage, provenance completeness, claim calibration, negative-result retention, and the distribution of responsibility between agents and human researchers.

\subsection{Competitor Landscape}
\label{sec:competitor-landscape}

Existing AI4R systems specialize in different stages of scientific work. AutoSurvey organizes literature retrieval, outline construction, and survey generation~\cite{wang2024autosurvey}. ResearchAgent and SciAgents ground research ideas in papers, academic graphs, or ontological knowledge graphs, and refine hypotheses through iterative agent interaction~\cite{baek2024researchagent,ghafarollahi2024sciagents}. AIDE, FunSearch, and AlphaEvolve search executable program spaces under external evaluators~\cite{jiang2025aide,romeraParedes2023funsearch,novikov2025alphaevolve}. The AI Scientist connects idea generation, implementation, experimentation, visualization, manuscript generation, and automated review~\cite{lu2024aiscientist}. Coscientist and A-Lab couple AI planning with robotic experimentation in chemistry and materials science~\cite{boiko2023coscientist,szymanski2023alab}. MLAgentBench, MLE-bench, and MLR-Bench provide evaluation environments for machine-learning research agents~\cite{huang2023mlagentbench,chan2024mlebench,chen2025mlrbench}.

Table~\ref{tab:competitor-matrix} summarizes the capabilities demonstrated in the corresponding publications. Program-search systems provide mature evaluator-driven optimization, autonomous laboratories provide direct physical execution, and end-to-end computational systems cover broader digital workflows. BLAZE concentrates on the connective structure across these stages: project-specific knowledge, hypothesis provenance, execution records, claim-evidence links, review closure, and explicit human checkpoints.

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{0.8}
\caption{Capability coverage of representative AI4R systems. \textbf{P}: primary; \textbf{S}: secondary or partial; \textbf{R}: roadmap; --: not reported as a principal capability.}
\label{tab:competitor-matrix}
\small
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\textbf{System} & \textbf{Lit.} & \textbf{Idea} & \textbf{Exec.} & \textbf{Write} &
\textbf{Review} & \textbf{Physical} & \textbf{Prov.} & \textbf{Human} \\
\midrule
AutoSurvey & \textbf{P} & -- & -- & \textit{S} & -- & -- & \textit{S} & -- \\
ResearchAgent / SciAgents & \textbf{P} & \textbf{P} & \textit{S} & -- & \textit{S} & -- & \textit{S} & -- \\
AIDE / FunSearch / AlphaEvolve & -- & \textit{S} & \textbf{P} & -- & -- & -- & \textit{S} & -- \\
The AI Scientist & \textit{S} & \textbf{P} & \textbf{P} & \textbf{P} & \textbf{P} & -- & \textit{S} & \textit{S} \\
Coscientist / A-Lab & \textit{S} & \textbf{P} & \textbf{P} & -- & -- & \textbf{P} & \textit{S} & \textit{S} \\
\textbf{BLAZE} & \textbf{P} & \textbf{P} & \textbf{P} & \textbf{P} & \textbf{P} & \textbf{R} & \textbf{P} & \textbf{P} \\
\bottomrule
\end{tabular}%
}
\end{table*}

Internal comparison materials provide additional positioning against AutoSOTA, FARS, ARIS, and EvoScientist. AutoSOTA shows stronger performance on large-scale, leaderboard-oriented optimization, while the current BLAZE cases are concentrated on auditable research loops for method development, traditional machine learning, lightweight computer vision, and interdisciplinary modeling. FARS produced a focused optimization direction in the ice-shelf task; the corresponding BLAZE package additionally retained baseline reproduction, experiment manifests, repeated-run results, review actions, unresolved work, and manuscript-level claim boundaries. ARIS and EvoScientist remain relevant comparators for idea generation and leaderboard-style exploration under aligned datasets, prompts, evaluation protocols, and budgets.

The comparison distinguishes stage breadth from stage maturity. Coverage of a research phase does not imply equivalent execution depth, and a specialized system may outperform a lifecycle platform within its target domain. BLAZE is therefore characterized by the density and continuity of its research artifacts rather than by a single aggregate capability score.

\subsection{Evidence Base and Evaluation Dimensions}
\label{sec:evidence-base}

The current evidence includes at least three complete idea-generation funnels, six representative experiment-planning or execution cases, and two \texttt{review-lite} revision chains. The retained artifacts include source records, candidate proposals, experiment plans, configurations, trial logs, JSON/CSV results, review assessments, action items, pending-work ledgers, route audits, and manuscript revisions.

Five dimensions organize the analysis. \textit{Execution coverage} measures whether a research plan reaches reproducible runs, repeated trials, or review-driven follow-up. \textit{Provenance completeness} measures whether reported results remain linked to data, configurations, logs, and comparison targets. \textit{Claim calibration} examines whether the language of a conclusion matches the strength and scope of its evidence. \textit{Negative-result retention} records failed runs, weaker variants, and stronger counter-baselines rather than preserving only the best result. \textit{Human governance} identifies the decisions that remain subject to researcher approval, including task scope, experimental boundaries, final claims, and submission.

The available traces show different workflow profiles. A single LLM is effective for drafting and local analysis but does not independently produce a reproducible experiment chain. Retrieval- and tool-enhanced models can complete literature, reproduction, or tuning fragments, while cross-stage coordination and claim boundaries remain largely manual. Full BLAZE connects reproduction, ideation, execution, review, and writing through persistent artifacts. Human work shifts toward objective definition, evaluation-boundary decisions, unresolved-risk assessment, and final approval.

\subsection{Cross-Scenario Internal Results}
\label{sec:cross-scenario}

Table~\ref{tab:case-studies} consolidates the currently supported numerical results. The cases span lightweight computer vision, multimodal identification, engineering--AI modeling, and review-driven method revision.

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{0.85}
\caption{Cross-scenario internal results. TF: test-feedback optimization; Scoped: restricted evidence scope; Ctrl.: stronger control retained.}
\label{tab:case-studies}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.18}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\textbf{Case} & \textbf{Protocol} & \textbf{Main result} & \textbf{Scope} \\
\midrule
TinySAM & Clean reproduction + TF tuning & \textbf{$42.2 \rightarrow 42.4$ AP; $+0.2$; $+0.47\%$} & TF \\
MDReID & RGBNT201 + TF tuning & \textbf{$77.5 \rightarrow 81.4$ mAP; $+3.9$; $+5.03\%$} & TF \\
Ice-shelf PINN & PCS repeated-run study & \textbf{$36$ seeds; $7.2/10$ review} & Scoped \\
Multi-view learning & $7$ datasets; $3$ seeds; $500$ epochs & \textbf{$42/42$ conditions $>$ zero-padding} & Ctrl. \\
\bottomrule
\end{tabular}%
}
\end{table*}

TinySAM reached AP $42.2$ under clean reproduction and AP $42.4$ after loose test-feedback optimization. The absolute gain of $0.2$ AP, or $0.47\%$ relative, mainly demonstrates successful reproduction and local tunability. The retained report separates the clean result, tuned configuration, trial history, and parameter changes, preventing the optimized value from being interpreted as independent held-out generalization.

MDReID increased from $77.5$ to $81.4$ mAP on RGBNT201, corresponding to a $3.9$-point or $5.03\%$ relative gain. The larger improvement indicates substantial task-specific optimization capacity. Its evidence boundary remains the same as TinySAM: the search used test feedback, and the resulting score is reported as test-feedback optimized rather than as a new independent benchmark result.

The ice-shelf PINN study completed a repeated-run PCS analysis over $36$ seeds. The associated \texttt{review-lite-v6} assessment assigned $7.2/10$ and retained unresolved ablation, robustness, and uncertainty-quantification tasks. The resulting claim is restricted to the reduced-budget constant-$B$ setting. The study therefore provides repeated-run support for a scoped detector claim while preserving the experimental work required for broader conclusions.

The multi-view learning study evaluated seven datasets, three random seeds, and 500 training epochs. The selected imputation-confidence variant outperformed zero-padding in all $42$ missing-plus-conflict conditions. This consistency supports the selected direction within the tested protocol. External-mask and available-view-mask controls remained stronger, changing the final interpretation from a universally superior mechanism to a promising direction with explicit counter-evidence and an incomplete official-SOTA comparison.

Across the four cases, the numerical evidence falls into two distinct classes. TinySAM and MDReID measure local optimization under test feedback, whereas the ice-shelf and multi-view cases provide broader within-protocol evidence through repeated seeds or multiple experimental conditions. Maintaining this distinction prevents heterogeneous results from being merged into a single performance claim.

\subsection{Workflow and Component Analysis}
\label{sec}

BLAZE's main advantage lies in evidence density rather than uniform metric superiority. Each result remains linked to its sources, configuration, execution logs, comparison target, review status, and claim boundary. The knowledge base supports literature grounding, baseline selection, and novelty checks; socialized review exposes missing baselines, metric mismatches, robustness gaps, and unsupported generalization; and the claim--evidence graph constrains manuscript statements to verified sources and results. TinySAM and MDReID remain labeled as test-feedback optimization, the ice-shelf claim is restricted to its validated setting, and the multi-view result preserves both its $42/42$ advantage over zero-padding and the stronger mask-based controls. Failed runs and negative results are also retained to distinguish implementation failure from hypothesis failure and reduce cherry-picking.

\subsection{Resource Profile, Human Governance, and Evidence Scope}
\label{sec}

BLAZE requires more retrieval, execution, review, and auditing than a single LLM, but reduces manual coordination across research stages and produces reusable, traceable artifacts. Agents support hypothesis generation, code execution, result aggregation, blocker detection, and revision drafting, while humans retain authority over research scope, protocol validity, claim strength, ethics, authorship, and submission. The current evidence supports competitor positioning, workflow analysis, component-level observations, and four traceable cases, while also defining clear limits: AutoSOTA may remain stronger on large-scale leaderboard optimization, test-feedback gains do not establish independent generalization, physical experimentation is not yet implemented, and broader robustness claims require additional experiments.

==> Related_Work/2.5-2.6.tex <==
\subsection{From Code Execution to End-to-End Research Automation}
\label{sec:execution-to-e2e}

In recent years, AI research assistance has evolved from language-only interaction into executable scientific work and end-to-end automation. Coding agents such as AIDE~\cite{jiang2025aide}, FunSearch~\cite{romeraParedes2023funsearch}, and AlphaEvolve~\cite{novikov2025alphaevolve} formulate machine learning engineering as exploration in code space, optimizing programs through external evaluators. This operational burden is further formalized by benchmarks like MLAgentBench~\cite{huang2023mlagentbench} and MLE-bench~\cite{chan2024mlebench}. Extending along this trajectory, systems such as The AI Scientist~\cite{lu2024aiscientist}, Agent Laboratory~\cite{schmidgall2025agentlab}, and MLR-Bench~\cite{chen2025mlrbench} attempt to coordinate the entire computational research loop—generating ideas, running experiments, writing drafts, and conducting automated reviews.

While these systems demonstrate that the research process can be decomposed into machine-operable stages, they all share a critical limitation: execution is not equivalent to scientific validity. An agent may successfully run code to optimize a metric or generate a fluent draft, yet it still struggles to test relevant hypotheses or compare against consistent baselines. For research, the decisive signal cannot merely be a successfully compiled script or a number on a leaderboard; it must be an evidence-supported claim explaining why a method works, when it fails, and what evidence justifies the conclusion. Thus, the frontier question in AI4R has shifted from automating research steps to ensuring that every step in the automated research process is grounded in solid experimental evidence.

BaiZe addresses this gap by operating not as a text-generation tool, but as an evidence-constrained research organization workflow. It decouples the product pillars that are often conflated in opaque demonstration pipelines. The knowledge base provides domain context; the \tool{id-pipeline} ensures evidence-grounded idea discovery; and the AutoPaper module translates these ideas into an experiment graph rather than isolated scripts. By utilizing distinct stages with strict scientific boundaries—such as \tool{auto-baseline} for auditable reproductions, \tool{idea-validation} for testing main results, \tool{benchmark-optimize} and \tool{benchmark-optimize-loose} for clearly delineated tuning, and \tool{review-lite} for deferred ablations—BaiZe binds executable work directly to research hypotheses.

This modular design ensures that every experiment node is traceable to a specific claim. Particularly during rigorous conference rebuttal phases or when managing complex configurations for multi-agent experiments, this transparency prevents massive computational waste and allows researchers to conduct highly targeted ablation studies with significant scientific value. Finally, considering the ethical implications of automated science, BaiZe treats the review stage as a weighted human-AI collaborative process~\cite{liang2024llmfeedback,gu2024llmjudge}. The goal is to reduce friction in responsible research rather than remove researchers from the loop, ensuring that human authors retain ultimate scientific responsibility.

==> Related_Work/2.5.tex <==
\subsection{AI Coding, Experiment Execution, and Machine Learning Engineering Agents}
\label{sec:ai-coding-experiment-agents}

AI coding and experiment-execution agents move research assistance from language-only interaction into executable scientific work. Instead of treating a model output as the final artifact, these systems place the model inside a loop: generate code, run the code, observe errors or metrics, revise the candidate, and repeat. AIDE formulates machine learning engineering as exploration in code space, where candidate solutions are generated, executed, and improved through a search process over programs~\cite{jiang2025aide}. FunSearch similarly combines language-model program proposal with an evaluator, showing that program search can produce verifiable discoveries in mathematics and algorithms~\cite{romeraParedes2023funsearch}. AlphaEvolve extends this direction by using a coding agent for scientific and algorithmic discovery, again emphasizing that the decisive signal is not fluent explanation but executable improvement under an external evaluator~\cite{novikov2025alphaevolve}.

This line of work is important for AI4R because it turns test-time computation into research labor. In traditional machine-learning research, large amounts of time are spent on code repair, data loading, training scripts, hyperparameter sweeps, and managing complex configurations for multi-agent frameworks or comparative experiments. Machine-learning-agent benchmarks make this operational burden explicit. MLAgentBench evaluates language agents on machine-learning experimentation tasks~\cite{huang2023mlagentbench}, while MLE-bench evaluates machine-learning agents on competition-style engineering tasks~\cite{chan2024mlebench}. However, existing systems typically lack a unified knowledge base, socialized deliberation, an experiment evidence graph, human governance, and cross-stage knowledge sedimentation. An agent may be able to run code and improve a score, yet still fail to preserve the scientific meaning of the experiment. For research, the object is not only a number on a leaderboard; it is a supported claim about why a method works, when it fails, and what evidence justifies the conclusion.

For BaiZe, this distinction defines the role of experimentation inside the system. The AutoPaper module operates not as a text-generation tool, but as a research organization workflow according to evidences. It translates ideas into an experiment graph rather than isolated scripts, utilizing distinct stages with strict scientific boundaries.The AutoPaper workflow uses stages such as \tool{auto-baseline}, \tool{idea-validation}, \tool{benchmark-optimize}, and \tool{review-lite}; these are not merely engineering utilities. They are intended to bind executable work to a research hypothesis. \tool{auto-baseline} establishes an auditable baseline reproduction from a paper and repository. \tool{idea-validation} converts an \tool{IDEA\_REPORT.md} or an \tool{id-pipeline} handoff into grouped runnable experiments. \tool{benchmark-optimize} and \tool{benchmark-optimize-loose} explore score-improving configurations under different integrity constraints, while \tool{review-lite} runs deferred ablations and checks obvious blockers. The scientific contribution of such a pipeline does not lie in automating code alone, but in making each experiment node traceable to a question, a baseline, a metric, a log, and a manuscript claim.

The remaining challenge is that execution is not equivalent to validity. An agent can optimize the wrong metric, misread a log, compare against an inconsistent baseline, or silently change the evaluation protocol. BaiZe therefore treats execution as one component of a larger evidence system. Code-generation success must be evaluated together with baseline fidelity, dataset and metric consistency, random-seed stability, ablation coverage, and claim support. This is the key gap between generic coding agents and a research infrastructure: the latter must organize execution as evidence, not as isolated automation.

==> Related_Work/2.6.tex <==
\subsection{End-to-End AI Research Automation}
\label{sec:end-to-end-ai-research}

End-to-end AI research automation asks whether an AI system can coordinate the entire computational research loop: generate ideas, check novelty, implement experiments, analyze results, write a paper, and sometimes review the generated paper. The AI Scientist is a representative system in this direction, demonstrating a pipeline for idea generation, experiment execution, paper writing, and automated review~\cite{lu2024aiscientist}. Agent Laboratory similarly frames LLM agents as research assistants that can participate in a broader research workflow~\cite{schmidgall2025agentlab}. MLR-Bench evaluates agents on open-ended machine-learning research, making the full workflow itself a benchmark object rather than evaluating only individual subskills~\cite{chen2025mlrbench}.

These systems show that the research process can be decomposed into machine-operable stages. Their value is not limited to writing drafts faster; they make it possible to study the failure modes of AI research labor. Idea generation may be shallow even when the paper is fluent. Experiments may run but fail to test the relevant hypothesis. A method may improve a metric without constituting a publishable contribution. Automated review may identify surface-level issues while missing the human judgment required for scientific responsibility. Thus, the frontier question is shifting from ``Can AI complete a sequence of research steps?'' to ``Can an AI-assisted organization make each step accountable to knowledge, evidence, and human judgment?''

BaiZe is positioned at this second level. Its architecture separates product pillars that are often fused into a single demonstration pipeline. The knowledge base provides literature, author, institution, venue, and trend context; the \tool{id-pipeline} provides evidence-grounded idea discovery through stages such as \tool{id-gap-discovery}, \tool{id-cross-discussion}, \tool{id-evidence-confirmation}, \tool{id-novelty-check}, and \tool{id-convergence}; AutoPaper then turns selected ideas into reproducible experiments, review loops, and manuscripts through named stages such as \tool{auto-baseline}, \tool{idea-validation}, \tool{review-lite}, \tool{auto-review-loop}, and \tool{paper-writing}. This modularity matters because the user may need to inspect, pause, rerun, or replace a stage without losing the provenance of the whole research process.Particularly during rigorous conference rebuttal phases or when managing complex configurations for multi-agent experiments, this transparency can prevent massive waste of computational resources and allow researchers to conduct targeted ablation experiments with high scientific significance.

End-to-end automation also raises ethical and institutional questions. Systems that can produce full papers could increase the burden on reviewers if they are used to generate low-value submissions. Recent work on LLM-based review and feedback suggests that models can provide useful structured comments, but also that such feedback cannot substitute for human academic responsibility~\cite{liang2024llmfeedback,gu2024llmjudge}. BaiZe therefore treats review as a weighted human-AI process rather than as a fully automated gate. The goal is to reduce friction in responsible research, not to remove the researcher from the loop.
